RunPHI: Enabling Mixed-criticality Containers via Partitioning Hypervisors in Industry 4.0

Orchestration systems are becoming a key component to automatically manage distributed computing resources in many fields with criticality requirements like Industry 4.0 (I4.0). However, they are mainly linked to OS-level virtualization, which is known to suffer from reduced isolation. In this paper, we propose RunPHI with the aim of integrating partitioning hypervisors, as a solution for assuring strong isolation, with OS-level orchestration systems. The purpose is to enable container orchestration in mixed-criticality systems with isolation requirements through partitioned containers.

==> tex/soa_table.tex <==
\begin{table}[ht]
\centering
\caption{State-of-the-art solutions for partitioned containers.}
\label{tab:table1}
\footnotesize                       % used font size
\resizebox{\linewidth}{!}{%
\sffamily \setstretch{0.50}
%\begin{tabular}{|>{\centering\columncolor{LightCyan}}p{2cm}|>{\centering}p{2.5cm}|>{\centering}p{2.5cm}|>{\centering}p{2.5cm}|}
\begin{tabular}{C{2cm}C{2cm}C{2cm}C{3cm}}
\hline 
\rowcolor{LightCyan}
 \textsf{\textbf{Solution}} & \textsf{\textbf{Type}} & \textsf{\textbf{Hypervisor}} & \textsf{\textbf{Orchestration}}\tabularnewline
\hline 
\hline 
\textsf{\textbf{vSphere (VIC) \cite{vic}}} & \textsf{ VMs and Containers} & \textsf{ESXi} & \textsf{VMware Orchestrator}\tabularnewline
\hline 
\textsf{\textbf{KubeVirt \cite{kubevirt}}} & \textsf{ VMs and Containers} & \textsf{KVM} & \textsf{ Kubernetes}\tabularnewline
\hline 
\textsf{\textbf{gVisor \cite{gvisor}}} & 
\rowcolor{LightGray}\textsf{ Application kenel} & \textsf{KVM} & \textsf{ Kubernetes/Docker}\tabularnewline
\hline 
\textsf{\textbf{Nabla Container \cite{nabla_ibm}}} &
\rowcolor{LightGray}\textsf{ Unikernels} & \textsf{Nabla Tender (KVM)} & \textsf{ Docker}\tabularnewline
\hline 
\textsf{\textbf{KataContainer \cite{kata_containers}}} &
\rowcolor{Gray}\textsf{ Light VMs} & \textsf{KVM (Firecracker, ...)} & \textsf{ Kubernetes/Docker}\tabularnewline
\hline 
\textsf{\textbf{RunX \cite{runx}}} & 
\rowcolor{Gray}\textsf{ Light VMs} & \textsf{XEN} & \textsf{ Kubernetes/Docker}\tabularnewline
\hline 
\textsf{\textbf{RunPHI}} & 
\rowcolor{Gray}\textsf{ Light VMs} & \textsf{Partitioning Hypervisors} & \textsf{ Kubernetes/Docker}\tabularnewline
\hline 
\end{tabular}}
\end{table}



